SampleNet: Differentiable Point Cloud Sampling

There is a growing number of tasks that work directly on point clouds. As the size of the point cloud grows, so do the computational demands of these tasks. A possible solution is to sample the point cloud first. Classic sampling approaches, such as farthest point sampling (FPS), do not consider the downstream task. A recent work showed that learning a task-specific sampling can improve results significantly. However, the proposed technique did not deal with the non-differentiability of the sampling operation and offered a workaround instead. We introduce a novel differentiable relaxation for point cloud sampling that approximates sampled points as a mixture of points in the primary input cloud. Our approximation scheme leads to consistently good results on classification and geometry reconstruction applications. We also show that the proposed sampling method can be used as a front to a point cloud registration network. This is a challenging task since sampling must be consistent across two different point clouds for a shared downstream task. In all cases, our approach outperforms existing non-learned and learned sampling alternatives. Our code is publicly available at https://github.com/itailang/SampleNet.

==> figures/reconstruction/failure_vis_matplot.tex <==
\begin{figure}[htb!]
\begin{center}
\begin{tabular}{ c c c}
\includegraphics[width=0.28\linewidth]{figures/reconstruction/matplot/airplane_328_input_pc.png} &
%\includegraphics[width=0.28\linewidth]{figures/reconstruction/matplot/airplane_328_samp_spnet64.png} &
\includegraphics[width=0.28\linewidth]{figures/reconstruction/matplot/airplane_328_samp_only_spnet64.png} &
%\includegraphics[width=0.28\linewidth]{figures/reconstruction/matplot/airplane_328_samp_fps64.png} \\
\includegraphics[width=0.28\linewidth]{figures/reconstruction/matplot/airplane_328_samp_only_fps64.png} \\
\includegraphics[width=0.28\linewidth]{figures/reconstruction/matplot/airplane_328_rcon_input.png} &
\includegraphics[width=0.28\linewidth]{figures/reconstruction/matplot/airplane_328_rcon_spnet64.png} &
\includegraphics[width=0.28\linewidth]{figures/reconstruction/matplot/airplane_328_rcon_fps64.png} \\
Complete & \SPNet & FPS \\
%NRE = 1.00 &
%NRE = 1.98 &
%NRE = 1.25 \\
\end{tabular}
%\caption{{\bfseries A failure example.} Top row: complete input with 2048 points, input with 64 \SPNet points (in Purple), input with 64 FPS points (in Magenta). Bottom row: reconstruction from complete input and from corresponding sampled points. In this case, uniform sampling by FPS yields better reconstruction result.}
\caption{{\bfseries A failure example.} Top row: complete input with 2048 points, 64 \SPNet points (in Purple), 64 FPS points (in Magenta). Bottom row: reconstruction from complete input and from corresponding sampled points. In this case, uniform sampling by FPS is preferred.}
\label{fig:failure_vis}
\end{center}
\end{figure}


==> figures/reconstruction/rcon_vis_matplot.tex <==
\begin{figure}[htb!]
\begin{center}
\begin{tabular}{ c c c c }
\includegraphics[width=0.19\linewidth]{figures/reconstruction/matplot/chair_558_input_pc.png} &
\includegraphics[width=0.19\linewidth]{figures/reconstruction/matplot/chair_558_samp_spnet64.png} &
\includegraphics[width=0.19\linewidth]{figures/reconstruction/matplot/chair_558_samp_snet64.png} &
\includegraphics[width=0.19\linewidth]{figures/reconstruction/matplot/chair_558_samp_fps64.png} \\
\includegraphics[width=0.19\linewidth]{figures/reconstruction/matplot/chair_558_rcon_input.png} &
\includegraphics[width=0.19\linewidth]{figures/reconstruction/matplot/chair_558_rcon_spnet64.png} &
\includegraphics[width=0.19\linewidth]{figures/reconstruction/matplot/chair_558_rcon_snet64.png} &
\includegraphics[width=0.19\linewidth]{figures/reconstruction/matplot/chair_558_rcon_fps64.png} \\
%NRE = 1.00 &
%NRE = 1.18 &
%NRE = 2.26 &
%NRE = 3.30 \\
%\\
\includegraphics[width=0.20\linewidth]{figures/reconstruction/matplot/car_593_input_pc.png} &
\includegraphics[width=0.20\linewidth]{figures/reconstruction/matplot/car_593_samp_spnet64.png} &
\includegraphics[width=0.20\linewidth]{figures/reconstruction/matplot/car_593_samp_snet64.png} &
\includegraphics[width=0.20\linewidth]{figures/reconstruction/matplot/car_593_samp_fps64.png} \\
\includegraphics[width=0.20\linewidth]{figures/reconstruction/matplot/car_593_rcon_input.png} &
\includegraphics[width=0.20\linewidth]{figures/reconstruction/matplot/car_593_rcon_spnet64.png} &
\includegraphics[width=0.20\linewidth]{figures/reconstruction/matplot/car_593_rcon_snet64.png} &
\includegraphics[width=0.20\linewidth]{figures/reconstruction/matplot/car_593_rcon_fps64.png} \\
%NRE = 1.00 &
%NRE = 1.20 &
%NRE = 1.57 &
%NRE = 1.89 \\
%\\
Complete & \SPNet & S-NET & FPS \\
\end{tabular}
\caption{{\bfseries Reconstruction from sampled points.} Top and third rows: complete input point cloud of 2048 points, input with 64 \SPNet points (in Purple), input with 64 S-NET points (in Green), input with 64 FPS points (in Magenta). Second and bottom rows: reconstructed point cloud from the input and the corresponding sample. Reconstructing from \SPNet points better preserves the input shape and is similar to the reconstruction from the complete input.}
\label{fig:rcon_vis}
\end{center}
\end{figure}

